Experimental Study of Concise Representations of Concepts and Dependencies

In this paper we are interested in studying concise representations of concepts and dependencies, i.e., implications and association rules. Such representations are based on equivalence classes and their elements, i.e., minimal generators, minimum generators including keys and passkeys, proper premises, and pseudo-intents. All these sets of attributes are significant and well studied from the computational point of view, while their statistical properties remain to be studied. This is the purpose of this paper to study these singular attribute sets and in parallel to study how to evaluate the complexity of a dataset from an FCA point of view. In the paper we analyze the empirical distributions and the sizes of these particular attribute sets. In addition we propose several measures of data complexity, such as distributivity, linearity, size of concepts, size of minimum generators, for the analysis of real-world and synthetic datasets.

==> Misc/abstract.tex <==
\begin{abstract}
Concise representations of concepts and dependencies (implications and association rules), such as minimal generators, minimum generators (keys and passkeys, respectively) and pseudo-intents are well studied from the computational point of view, however their statistical properties are still to be studied. A study of this sort can shed some light on  complexity of data for FCA-based approaches. Here we analyze empirical distributions of sizes of concise representations and propose several measures of data complexity tailored for methods based on concepts and dependencies.

\keywords{Formal Concept Analysis  \and Concise representations \and Data complexity.}
\end{abstract}

==> Misc/background_simpest_example.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Theoretical Background}

\subsection{Classes of descriptions}
Here we recall basic FCA definitions related to concepts, dependencies, and their minimal representations. After that we illustrate the definitions with a toy example.

Given a formal context $K = (G, M, I)$ and prime operators:
\begin{align}
    A' &= \{m \in M \mid \forall g \in A: gIm \}, \quad A \subseteq G \\
    B' &= \{g \in G \mid \forall m \in B: gIm \}, \quad B \subseteq M
\end{align}

In what follows we illustrate the description classes definitions using the toy formal context from Table \ref{tbl:toy_context}, where the set of objects $G = \{g_1, g_2\}$, and the set of attributes $M = \{a, b, c, d\}$.

\begin{table}
    \caption{An example formal context}
    \centering
    \label{tbl:toy_context}
    \begin{tabular}{r|llll|}
        %\toprule
        {} &  a &  b &  c & d \\
        \midrule
        $g_1$ &    &    &  X &   \\
        $g_2$ &  X &  X &    &   \\
        \bottomrule
    \end{tabular}
\end{table}


\begin{definition}[Intent (closed description)]
A subset of attributes $B \subseteq M$ is an intent (is closed) iff $B'' = B$.
\end{definition}

An example (acc. to Table \ref{tbl:toy_context}): $B = \{a, b\}$ is an intent since it is a maximal subset of attributes that describes the subset of objects $B' = \{g_1\}, B'' = \{a, b\} = B$.


\begin{definition}[Pseudo-intent]
A subset of attributes $P \subseteq M$  is a pseudo-intent iff:
\begin{enumerate}
    \item $P \neq P''$
    \item $Q'' \subset P$ for every pseudo-intent $Q \subset P$
\end{enumerate}
Pseudo-intents are premises of implications of the cardinality-minimal implication base, called Duquenne-Guigues or canonical base, or stembase.

\end{definition}

An example (acc. to Table \ref{tbl:toy_context}): elements of a set $\big\{\{a\}, \{b\}, \{d\}, \{a, b,c\}\big\}$ are pseudo-intents, since:
\begin{itemize}
    \item $\{a\}, \{b\}, \{d\}$ are the minimal non-closed subsets of attributes, and
    \item $\{a,b,c\}$ is both non-closed and contains the closure $\{a, b\}$ of pseudo-intents $\{a\}$ and $\{b\}$.
\end{itemize} 

\begin{definition}[Proper premise]
A set of attributes $A \subseteq M$ is a proper premise iff:
$$A \cup \bigcup_{n \in A} \left( A \setminus \{n\} \right)'' \neq A''$$
\end{definition}
Proper premises are premises of so-called direct (or proper-premise) base of implications, from which one obtains all implications with a single application of Armstrong rules.

An example (acc. to Table \ref{tbl:toy_context}): $Q = \{a, c\}$ is a proper premise since the union of $Q$ with the closures of its subsets does not result in the closure of $Q$: $\{a, c\} \cup \{a\}'' \cup \{c\}'' = \{a, c\} \cup \{a ,b \} \cup \{c\} = \{a, b, c\} \neq \{a,b,c,d\}$.

\begin{definition}[Generator]
A set of attributes $D \subseteq M$ is a generator iff $\exists B \subseteq M: D'' = B$.
\end{definition}
Every subset of attributes is a generator of a concept intent. A generator is called non-trivial if it is not closed.

An example (acc. to Table \ref{tbl:toy_context}): $D = \{b,d\}$ is a generator, since there is an intent $B = \{a,b,c,d\} = D''$.


\begin{definition}[Minimal generator, key]
A set of attributes $D \subseteq M$ is a minimal generator (or key) of $D''$ iff:
$$ \nexists m \in D: (D \setminus \{m\})'' = D'' $$
\end{definition}
A minimal generator is inclusion minimal in the equivalence class of subsets of attributes having the same closure. Every proper premise is a minimal generator, however the converse does not hold in general.

An example (acc. to Table \ref{tbl:toy_context}): $D = \{a, c\}$ is a minimal generator (and a proper premise) since none of its subparts $\{a\}, \{c\}$ generates the same intent $D''$; $D = \{c\}$ is a minimal generator (though not a proper premise) since it is the minimal set of attributes that generates an intent $D'' = \{c\}$.

\begin{definition}[Minimum generator, passkey]
A set of attributes $D \subseteq M$ is a minimum generator iff:
\begin{enumerate}
    \item $D$ is a minimal generator
    \item $\nexists E \subseteq M$, s.t. $E$ is a minimal generator of $D''$ and $|E| < |D|$.  %% E.D. This line previously stated that $|E| > |D|$. This is wrong, right?
\end{enumerate}
\end{definition}
A minimum generator (a passkey) is cardinality-minimal in the equivalence class of subsets of attributes having the same closure. 
In~\cite{MakhalovaBKN22} the size of a maximal passkey of a context was studied as an important index of the context complexity. 

An example (acc. to Table \ref{tbl:toy_context}): $D= \{d\}$ is a minimum generator of an intent $\{a,b,c,d\}$ since the only smaller subset of attributes $E = \emptyset$ generates another intent $D''\neq E''$; $D = \{a, c\}$ is not a minimum generator of $\{a,b,c,d\}$ since there is a subset $E = \{d\}$ with the same intent $E''=D''$.

Finally, let us illustrate all definitions at once. To do so, we form the context of description classes $(2^M, M_d, I_d)$, where $M_d = \{\mathrm{passkey}, \mathrm{key}, \mathrm{proper\ premise}, \ldots\}$, and $I_d$ defines whether a subset of attributes from $2^M$ belongs to a description class in $M_d$. The concept lattice of this context (without the empty bottom concept) is shown in Figure \ref{fig:descr_lattice_toy_context}.

\begin{figure}[h!]
  \includegraphics[width=\textwidth]{fig/toy_description_lattice.png}
  \caption{Lattice of description classes on example context}
  \label{fig:descr_lattice_toy_context}
\end{figure}

\subsection{Towards measuring data complexity}

When one speaks that data is complex it can mean many different things depending on the context. In particular, data can be claimed to be complex, if processing of it takes to much time, i.e., computational complexity of certain data processing procedure. Alternatively, one can claim that data is complex, if the result of the analysis is hard to interpret. The complexity of data can also be related to difficulty of solving other tasks with this data. In particular, if the data is used for solving supervised learning task, e.g., classification or regression, the complexity of the data can also be related to complexity of solving this task. Accordingly, it is quite hard to define data complexity in general terms.

If we think in the direction of the interpretability, then the size of the elements to interpret and the number of them are definitely important. In the ideal case, one would prefer a small number of small elements. Indeed, one rule of two attributes in the premise and one attribute in the conclusion are simpler to interpret, then 100 rules with tenth of attributes in the premise and dozens of attributes in the conclusion. Thus, it is natural to study how the number of elements are distributed w.r.t. their size. Moreover, in most of the cases larger numbers of elements are associated with computational complexity, thus controlling for the size and the number of elements is also a proxy to computational complexity.

It should also be mentioned that the number of elements is related to a so-called VC-dimension~\ref{} that measures the minimal size of the Boolean lattice all elements can be fitted to, i.e., the larger elements of has found, the larger the corresponding Boolean lattice size is expected.

Accordingly, we decided to count the number of concepts, pseudo-intents, proper premises, keys, and passkeys in order to grasp the complexity of the data. For all this elements, we also study the distribution of the element sizes.

Additionally, we decided to measure the lattice complexity with two new measures that are related to ``linearity'' of the lattice. Indeed, the most simple lattice  structure that we can imagine is a chain. It counterpart is Boolean lattice, i.e., the lattice with largest amount of connections and concepts. 
%We can definitely said that Boolean lattice is ``complex'', 
%since in terms of implications it is a trivial structure. Nevertheless, from the point of view of interpretability it can be considered complex. 
%
The first way to measure the closeness of the lattice to a chain is linearity index. We define the linearity index as the probability that two random concepts from the lattice are comparable.

\begin{definition}
    Given a lattice $\mathcal{L}$, the linearity index is defined as
    \begin{equation}
        \mathtt{LIN}(\mathcal{L}) = \frac{1}{|\mathcal{L}|}\underset{c_1,c_2 \in \mathcal{L}}{\sum} I(c_1 < c_2 \vee c_1 > c_2)
    \end{equation}
\end{definition}

The linearity index is maximized for a chain lattice and is minimized for the lattice of a nominal scale. This index does not directly measure how well the result is interpretable. One of the key interpretability property is the size of the element set. In particular, the size and the structure of the implication basis. One of the most simple structure for the implication basis can be found for distributive lattices. Accordingly, we define the distributivity index, the measures how close the lattice to distributive one.

\begin{definition}
    Given a lattice $\mathcal{L}$, the distributivity index is defined as
    \begin{equation}
        \mathtt{DIST}(\mathcal{L}) = \frac{1}{|\mathcal{L}|}\underset{i_1,i_2 \in Intents(\mathcal{L})}{\sum} I(i_1 \cup i_2 \in Intents(\mathcal{L})),
    \end{equation}
    where $Intents(\mathcal{L})$ is the set of intents for concepts form $\mathcal{L}$.
\end{definition}

The distributivity index is maximized for distributive lattices, including chain lattices, and is minimized for lattices of nominal scales. Although, it can be strange that lattices of nominal scales would be reported as complex, however from the point of view of implications they are not simple. In particular, any pair of attributes from such lattices would form a premise of an implication with nonempty conclusion. This introduce many implications to the basis that makes it hard to interpret the implication basis.

\subsection{Synthetic complex data}

In order to study different ways of measuring data complexity, we need to compare the behavior of different complexity indices for ``simple'' and ``complex'' data. However, beforehand we cannot know which dataset is complex. Accordingly, we will synthetically generate complex datasets and compare them with real-world data.

One way of generating complex data is randomization. Indeed, randomized data cannot be interpreted since any possible result is an artefact of the data. For randomized data we know before hand that there is no rules or concepts that has some meaning. So randomized data is a good data for being called ``complex''.

What randomization strategy should we use for generating such data. A natural way is making the randomized data similar in some sense to the real data it is compared to. First, it seems natural to fix the number of objects and attributes the same as they are in the real data. Moreover, the density of the context, i.e., the number of crosses, significantly influence the size and structure of the concept lattice. Thus, to make the randomized data similar to the real data it is natural to fix also the density of the data. It would give us the first randomization strategy, i.e., for any real dataset we can generate a randomized dataset with the same number of objects and attributes and with the same density as the real data. In this case, the crosses in the formal context would be randomly spread along the context ensuring that the final density is the same as in the corresponding real data. 

Let as exemplify this strategy for the context from Table~\ref{tbl:descr_lattice_bobross}. It has 8 objects and 9 attributes. In total, it has 35 crosses. Thus, any context that has 8 objects, 9 attributes and 35 crosses can be considered as a randomisation of it. In our first randomization strategy we fix that the probability of generating any such randomized context is equal.

The randomized formal contexts for such strategy where studied in~\ref{Borchmann2016}. The authors has found, that the correlation between the number of concepts and the number of pseudo-intents has a non-random structure suggesting that fixing density is not enough in order to generate randomized data which is similar to the real one.

Accordingly, we also study randomization strategy that fixes the number of objects having cross for every attributes. It can be done in the following way. A randomized context is generated attribute by attribute. The crosses in every column is put randomly and the number of crosses corresponds to the number of crosses in the corresponding attribute. So it can be considered as a permutation of crosses within every column in the context independently from other columns. Such a procedure corresponds to the zero hypothesis in statistical terms of independence between attributes. Although such randomization treats objects and attributes differently, this strategy correspond to typical cases of data analysis. Indeed, in typical datasets, objects are considered to observations that can be described with different attributes. In such cases the attributes are not fixed and could correspond to any hypothesis of the data analytic. Then, one is usually search for some relations between such attributes, and the the hypothesis of attribute independence is a natural zero-hypthesis for such settings. 

Let as exemplify the second strategy for the context from Table~\ref{tbl:descr_lattice_bobross}. The numbers of objects and attributes in the randomized context remain the same. Then a randomized context with the second strategy is any context that has 8 crosses for the first attribute, 2 crosses for the second attribute, 5 crosses for the 3rd attribute etc.

Finally, studying randomized data one should take into account that for one real dataset one can generate many randomized dataset with the same strategy. Thus, it is not enough to study just one random dataset for one real dataset. In order, to objectively estimate the behaviour of randomized dataset it is necessary to generate many of them and then estimate the distribution of a certain dataset characteristics within all randomized dataset.

In the next section we will try to study how different ways of measuring complexity of a dataset reflect the fact that complexity of random data should be higher than the complexity of the corresponding real data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








==> Misc/content.tex <==
\section{Introduction}

Data
\section{Theoretical Background}
\textcolor{orange}{E.D.: Just excerpts from the current experiments notebooks}
\subsection{Classes of descriptions}
Here we recall basic FCA definitions related to concepts, dependencies, and their minimal representations. After that we illustrate the definitions with a toy example.

Given a formal context $K = (G, M, I)$ and prime operators:
\begin{align}
    A' &= \{m \in M \mid \forall g \in A: gIm \}, \quad A \subseteq G \\
    B' &= \{g \in G \mid \forall m \in B: gIm \}, \quad B \subseteq M
\end{align}

\begin{definition}[Intent (closed description)]
A subset of attributes $B \subseteq M$ is an intent (is closed) iff $B'' = B$.
\end{definition}

\begin{definition}[Pseudo-intent]
A subset of attributes $P \subseteq M$  is a pseudo-intent iff:
\begin{enumerate}
    \item $P \neq P''$
    \item $Q'' \subset P$ for every pseudo-intent $Q \subset P$
\end{enumerate}
Pseudo-intents are premises of implications of the cardinality-minimal implication base, called Duquenne-Guigues or canonical base, or stembase.

\end{definition}

\begin{definition}[Proper premise]
A set of attributes $Q \subseteq M$ is a proper premise iff:
\begin{enumerate}
    \item $Q \subset M$
    \item $Q'' \neq Q$, and
    \item $ (Q \setminus \{n\})'' \neq Q \quad \forall n \in Q$
\end{enumerate}
\end{definition}
Proper premises are premises of so-called direct (or proper-premise) base of implications, from which one obtains all implications with a single application of Armstrong rules.

\begin{definition}[Generator]
A set of attributes $D \subseteq M$ is a generator iff $\exists B \subseteq M: D'' = B$.
\end{definition}
Every subset of attributes is a generator of a concept intent. A generator is called non-trivial if it is not closed.

\begin{definition}[Minimal generator, key]
A set of attributes $D \subseteq M$ is a minimal generator (or key) of $D''$ iff:
$$ \nexists m \in D: (D \setminus \{m\})'' = D'' $$
\end{definition}
A minimal generator is inclusion minimal in the equivalence class of subsets of attributes having the same closure. Every proper premise is a minimal generator, however the converse does not hold in general.

\begin{definition}[Minimum generator, passkey]
A set of attributes $D \subseteq M$ is a minimum generator iff:
\begin{enumerate}
    \item $D$ is a minimal generator
    \item $\nexists E \subseteq M$, s.t. $E$ is a minimal generator of $D''$ and $|E| > |D|$.
\end{enumerate}
\end{definition}
A minimum generator (a passkey) is cardinality-minimal in the equivalence class of subsets of attributes having the same closure. 
In~\cite{ijar2022} the size of a maximal passkey of a context was studied as an important index of the context complexity. 


Let us illustrate the aforementioned definition with the toy example: a shortened Mango formal context presented on Table \ref{tbl:short_mango_context}.
% ? Should we come up with the new name for the context? Since there is no mango object in it.

\begin{table}
    \caption{Shortened Mango formal context}
    \centering
    \label{tbl:short_mango_context}
    \begin{tabular}{r|llll}
        \toprule
        {} & oval & firm & green & blue \\
        \midrule
        egg      &    X &    X &       &      \\
        kiwi     &    X &      &     X &      \\
        plum     &    X &      &       &    X \\
        toy cube &      &    X &     X &      \\
        apple    &      &      &       &      \\
        \bottomrule
    \end{tabular}
\end{table}

Having only four attributes in Table \ref{tbl:short_mango_context}, we can enlist all sixteen subsets of these attributes. Doing so we test whether each subset of attributes satisfies the given definitions. Table \ref{tbl:short_mango_descriptions} shows these tests. 

\begin{table}
    \caption{Subsets of attributes of Shortened Mango formal context}
    \centering
    \label{tbl:short_mango_descriptions}
    \begin{tabular}{r||l|l|l|l|l}
        \toprule
        {} & closed description, & minimal generator, & minimum generator, & pseudo- & proper \\
        {Subset of attributes} &             intent &               key &           passkey & intent &  premise \\
        \midrule
        $\emptyset$             &                  X &                 X &                 X &               &                \\
        blue                 &                    &                 X &                 X &             X &              X \\
        green                &                  X &                 X &                 X &               &                \\
        oval                 &                  X &                 X &                 X &               &                \\
        firm                 &                  X &                 X &                 X &               &                \\
        blue,green           &                    &                 X &                 X &               &              X \\
        blue,oval            &                  X &                   &                   &               &                \\
        blue,firm            &                    &                 X &                 X &               &              X \\
        green,oval           &                  X &                 X &                 X &               &                \\
        green,firm           &                  X &                 X &                 X &               &                \\
        oval,firm            &                  X &                 X &                 X &               &                \\
        blue,green,oval      &                    &                   &                   &             X &                \\
        blue,green,firm      &                    &                   &                   &               &                \\
        blue,oval,firm       &                    &                   &                   &             X &                \\
        green,oval,firm      &                    &                 X &                   &             X &              X \\
        blue,green,oval,firm &                  X &                   &                   &               &                \\
        \bottomrule
    \end{tabular}
\end{table}




\section{Methods and Materials}

\subsection{Data complexity}


\section{Experiments}

\textcolor{orange}{E.D.: Just excerpts from emails}

We use 4 datasets:
\begin{itemize}
    \item "Live in water" \url{https://upriss.github.io/fca/examples.html}
    \item "Tea ladies" \url{https://upriss.github.io/fca/examples.html}
    \item "Lattice of lattice properties" \url{https://upriss.github.io/fca/examples.html}
    \item "Bob Ross episodes" \url{https://datahub.io/five-thirty-eight/bob-ross}
\end{itemize}

We decided answer the question in an empirical way. The experiment pipeline is as follows:
\begin{itemize}
    \item Given a context $K = (G, M, I)$, we iterate through all the possible descriptions (i.e. subsets of attributes, $2^M$) and check whether the description is closed, is a pseudo-intent, is a minimum generator, etc.;
    \item We construct a new "descriptions context" = $(2^M, \{ \mathrm{is\_closed}, \mathrm{is\_minimum\_generator}, \ldots \} )$; and
    \item Finally, we construct a "lattice of descriptions" over the "descriptions context".
\end{itemize}


\begin{figure}[h!]
  \includegraphics[width=\textwidth]{fig/Description_lattices_BobRoss.png}
  \caption{Lattice of descriptions for Bob Ross dataset}
  \label{fig:descr_lattice_bobross}
\end{figure}

\begin{table}
    \caption{Reduced formal context corresponding to lattice of descriptions for Bob Ross dataset}
    \label{tbl:descr_lattice_bobross}
    \begin{tabular}{r|lllllllll}
        \toprule
                   \# &        is &     is &    is &    is     &    is    &         is & is & is & is  \\
        descriptions & generator & closed & minimal & minimum & pseudo &  proper & key & passkey & intent \\
                  &        &  descr &     gen &     gen & intent & premise &  &      &     \\
        \midrule
                  67 &         X &      X &       X &       X &        &         &   X &       X &      X \\
                  45 &         X &      X &         &         &        &         &     &         &      X \\
                  41 &         X &        &       X &       X &      X &       X &   X &       X &        \\
                 125 &         X &        &       X &       X &        &       X &   X &       X &        \\
                   1 &         X &        &       X &         &      X &       X &   X &         &        \\
                  25 &         X &        &       X &         &        &       X &   X &         &        \\
                  33 &         X &        &         &         &      X &         &     &         &        \\
             1048239 &         X &        &         &         &        &         &     &         &        \\
        \bottomrule
    \end{tabular}
\end{table}



\begin{figure}[h!]
  \includegraphics[width=\textwidth]{fig/Description_lattices.png}
  \caption{Lattices of descriptions}
  \label{fig:descr_lattices}
\end{figure}

Figure \ref{fig:descr_lattice_bobross} shows that any two classes of descriptions may intersect if it is not restricted by their definition (e.g. a description can never be both an intent and a pseudo-intent). Figure \ref{fig:descr_lattices} represents the growth of a description lattice following the growth of the complexity of the corresponding formal context.
Table \ref{tbl:descr_lattice_bobross} provides the formal context representation of the description lattice from Figure \ref{fig:descr_lattice_bobross}.

The proportions of sizes of classes of descriptions are also should be taken into account. For example, given Bob Ross context with $20$ attributes, there are $2^{20}$ possible descriptions, but only $112$ of them are closed, and only $259$ of them are minimal generators. Thus the vast majority of the descriptions are "useless".

Given the experiments pipeline described in the previous sections, we have come up with various histograms for the each of the dataset. The histograms are shown on figures \ref{fig:hist_water}, \ref{fig:hist_tealadies}, \ref{fig:hist_lattices}, and \ref{fig:hist_bobross}.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{fig/hists_water.png}
    \caption{Histograms for "Live in water" dataset}
    \label{fig:hist_water}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{fig/hists_tealady.png}
    \caption{Histograms for "Tea ladies" dataset}
    \label{fig:hist_tealadies}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{fig/hists_lattice.png}
    \caption{Histograms for "Lattice of lattice properties" dataset}
    \label{fig:hist_lattices}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{fig/hists_BobRossShort.png}
    \caption{Histograms for "Bob Ross episodes" (first 20 attributes) dataset}
    \label{fig:hist_bobross}
\end{figure}


\section{Conclusion}

\section*{Acknowledgments}

@BOOK{Ganter:1999,
  title = {{Formal Concept Analysis: Mathematical Foundations}},
  publisher = {Springer-Verlag New York, Inc.},
  year = {1999},
  author = {Ganter, Bernhard and Wille, Rudolf},
  address = {Secaucus, NJ, USA},
  edition = {1st},
  isbn = {3540627715},
  owner = {Dmitry},
  timestamp = {2012.04.21}
}









==> Misc/header.tex <==
\title{Experimental Study of Concise Representations of Concepts and Dependencies
%\thanks{Supported by organization x.}
}
% If the paper title is too long for the running head, you can set
% an abbreviated paper title here
%
\author{
Aleksey Buzmakov\inst{1}\orcidID{0000-0002-9317-8785} \\
Egor Dudyrev\inst{2}\orcidID{0000-0002-2144-3308} \\
Sergei O. Kuznetsov\inst{2}\orcidID{0000-0003-3284-9001}\\
Tatiana Makhalova\inst{3}\orcidID{0000-0002-6724-3803} \\
Amedeo Napoli\inst{3}\orcidID{0000-0001-5236-9561} \\
}
%
\authorrunning{Aleksey Buzmakov, Egor Dudyrev, et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{
    \inst{1}%
    HSE University, Perm, Russia\\
    \inst{2}%
    HSE University, Moscow, Russia\\
    \inst{3}
    Université de Lorraine, CNRS, Inria, LORIA, F-54000 Nancy, France
}

%
\maketitle              % typeset the header of the contribution
%
